How is Exotics Produced ? Where to Search for it ?

On the basis of existing data, we suggest such a mechanism of production for exotic hadrons that can explain, at least qualitatively, why the Theta+-baryon is seen in some experiments and not in others. With our hypothesis, production of exotic hadrons is a new kind of hard processes. We also can propose new experiments to check (and confirm?) existence of exotics and to provide new important information about both exotic and conventional hadrons [The talk is based on the papers by Ya. Azimov, K. Goeke, and I. Strakovsky, Phys Rev D 76, 074013 (2007)]

==> MENU07macros.tex <==


%%%  useful macros for MENU proceedings articles:

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%  basic formatting macros:
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\def\Title#1{\begin{center} {\Large {\bf #1} } \end{center}}

%%  single-line equations:

\newcommand{\beq}{\begin{equation}}
\newcommand{\eeq}[1]{\label{#1}\end{equation}}
\newcommand{\eeqn}{\end{equation}}

%%  multiple-line equations  (use \CR as the carriage return):

\newcommand{\beqa}{\begin{eqnarray}}
\newcommand{\eeqa}[1]{\label{#1}\end{eqnarray}}
\newcommand{\eeqan}{\end{eqnarray}}
\newcommand{\CR}{\nonumber \\ }

%%  reference to an equation number:

\newcommand{\leqn}[1]{(\ref{#1})}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%  bibliographic entries   (use this or the SPIRES LaTeX output)


\def\Journal#1#2#3#4{{#1} {\bf #2}, #3 (#4)}
\def\add#1#2#3{{\bf #1}, #2 (#3)}

%% Some useful journal names

\newcommand{\NPB}{Nucl. Phys. B}
\newcommand{\PLB}{Phys. Lett.  B}
\newcommand{\PRL}{Phys. Rev. Lett.}
\newcommand{\PRD}{Phys. Rev. D}
\newcommand{\PR}{Phys. Rev.}
\newcommand{\ZPC}{Z. Phys. C}
\newcommand{\SJNP}{Sov. J. Nucl. Phys.}
\newcommand{\AnnP}{Ann. Phys.}
\newcommand{\JETPL}{JETP Lett.}
\newcommand{\LMP}{Lett. Math. Phys.}
\newcommand{\CMP}{Comm. Math. Phys.}
\newcommand{\PTP}{Prog. Theor. Phys.}
\newcommand{\NIM}{NIM}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%  sizing and bars

\newcommand{\st}{\scriptstyle}
\newcommand{\sst}{\scriptscriptstyle}
\newcommand{\overbar}[1]{\overline{#1}}
\let\littlebar=\bar
\let\bar=\overbar

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%  text-mode macros:

\newcommand{\etal}{{\it et al.}}
\newcommand{\ie}{{\it i.e.}}
\newcommand{\eg}{{\it e.g.}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%  expectation values:

\newcommand{\VEV}[1]{\left\langle{ #1} \right\rangle}
\newcommand{\bra}[1]{\left\langle{ #1} \right|}
\newcommand{\ket}[1]{\left| {#1} \right\rangle}
\newcommand{\vev}[1]{\langle #1 \rangle}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%  caligraphic letters (for matrix elements, luminosity, etc.)

\newcommand{\D}{{\cal D}}
\renewcommand{\L}{{\cal L}}
\newcommand{\M}{{\cal M}}
\newcommand{\A}{{\cal A}}
\renewcommand{\O}{{\cal O}}
\newcommand{\W}{{\cal W}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%  matrix operations and fractions:

\newcommand{\One}{{\bf 1}}
\newcommand{\hc}{{\mbox{\rm h.c.}}}
\newcommand{\tr}{{\mbox{\rm tr}}}
\newcommand{\half}{\frac{1}{2}}
\newcommand{\thalf}{\frac{3}{2}}

\newcommand{\Dslash}{\not{\hbox{\kern-4pt $D$}}}
\newcommand{\dslash}{\not{\hbox{\kern-2pt $\del$}}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%  high-energy physics terminology:

\newcommand{\Pl}{{\mbox{\scriptsize Pl}}}
\newcommand{\eff}{{\mbox{\scriptsize eff}}}
\newcommand{\CM}{{\mbox{\scriptsize CM}}}
\newcommand{\BR}{\mbox{\rm BR}}
\newcommand{\ee}{e^+e^-}
\newcommand{\sstw}{\sin^2\theta_w}
\newcommand{\cstw}{\cos^2\theta_w}
\newcommand{\mz}{m_Z}
\newcommand{\gz}{\Gamma_Z}
\newcommand{\mw}{m_W}
\newcommand{\mt}{m_t}
\newcommand{\gt}{\Gamma_t}
\newcommand{\gmu}{G_\mu}
\newcommand{\GF}{G_F}
\newcommand{\alphas}{\alpha_s}
\newcommand{\msb}{{\bar{\ssstyle M \kern -1pt S}}}
\newcommand{\lmsb}{\Lambda_{\msb}}
\newcommand{\ELER}{e^-_Le^+_R}
\newcommand{\EREL}{e^-_Re^+_L}
\newcommand{\ELEL}{e^-_Le^+_L}
\newcommand{\ERER}{e^-_Re^+_R}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%  supersymmetry:

\newcommand{\ch}[1]{\widetilde\chi^+_{#1}}
\newcommand{\chm}[1]{\widetilde\chi^-_{#1}}
\renewcommand{\ne}[1]{\widetilde\chi^0_{#1}}
\newcommand{\s}[1]{\widetilde{#1}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\def\vckm{V_{\rm CKM}}

\newcommand{\lsim} {\buildrel < \over {_\sim}}
\newcommand{\gsim} {\buildrel > \over {_\sim}}

